Weakly reversible mass-action systems with infinitely many positive steady states

We show that weakly reversible mass-action systems can have a continuum of positive steady states, coming from the zeroes of a multivariate polynomial. Moreover, the same is true of systems whose underlying reaction network is reversible and has a single connected component. In our construction, we relate operations on the reaction network to the multivariate polynomial occurring as a common factor in the system of differential equations.

==> fig-ell1-9squares.tex <==
\begin{tikzpicture}[scale=1.6]% was 1.9
\node at (0,-0.2) {\vphantom{.}};

\draw [step=1, gray, very thin] (0,0) grid (3.5,3.5);
\draw [ ->, black!70!white] (0,0)--(3.5,0);
\draw [ ->, black!70!white] (0,0)--(0,3.5);


%%% ORGANIZATION:
%%      -- (0,0) square
%%      -- (2,0) square
%%      -- (2,2) square
%%      -- (0,2) square
%%      -- (1,1) square
%%      -- X <--> 2X BOTTOM edge
%%      -- RIGHT edge
%%      -- TOP edge
%%      -- LEFT edge


\begin{scope}[shift={(0,0)}]
\node[inner sep=0,outer sep=1] (A) at (0,0)  {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (B) at (1,0) {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (C) at (1,1) {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (D) at (0,1) {\large \blue{$\bullet$}};

\draw[arrows={-stealth},very thick,blue,above, transform canvas={yshift=1.75pt}] (A) to node {$1$} (B);
\draw[arrows={-stealth},very thick,blue,below, transform canvas={yshift=-1.75pt}] (B) to node {$1$} (A);

\draw[arrows={-stealth},very thick,blue,right, transform canvas={xshift=1.75pt}] (C) to node {$11$} (B);
\draw[arrows={-stealth},very thick,blue,left, transform canvas={xshift=-1.75pt}] (B) to node {$2$} (C);

\draw[arrows={-stealth},very thick,blue,above, transform canvas={yshift=1.75pt}] (D) to node {$2$} (C);
\draw[arrows={-stealth},very thick,blue,below, transform canvas={yshift=-1.75pt}] (C) to node {$11$} (D);

\draw[arrows={-stealth},very thick,blue,left, transform canvas={xshift=-1.75pt}] (A) to node {$1$} (D);
\draw[arrows={-stealth},very thick,blue,right, transform canvas={xshift=1.75pt}] (D) to node {$1$} (A);
\end{scope}




\begin{scope}[shift={(2,0)}]
\node[inner sep=0,outer sep=1] (A) at (0,0)  {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (B) at (1,0) {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (C) at (1,1) {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (D) at (0,1) {\large \blue{$\bullet$}};

\draw[arrows={-stealth},very thick,blue,above, transform canvas={yshift=1.75pt}] (A) to node {$1$} (B);
\draw[arrows={-stealth},very thick,blue,below, transform canvas={yshift=-1.75pt}] (B) to node {$1$} (A);

\draw[arrows={-stealth},very thick,blue,left, transform canvas={xshift=-1.75pt}] (B) to node {$1$} (C);
\draw[arrows={-stealth},very thick,blue,right, transform canvas={xshift=1.75pt}] (C) to node {$1$} (B);

\draw[arrows={-stealth},very thick,blue,above, transform canvas={yshift=1.75pt}] (D) to node {$11$} (C);
\draw[arrows={-stealth},very thick,blue,below, transform canvas={yshift=-1.75pt}] (C) to node {$2$} (D);

\draw[arrows={-stealth},very thick,blue,left, transform canvas={xshift=-1.75pt}] (A) to node {$2$} (D);
\draw[arrows={-stealth},very thick,blue,right, transform canvas={xshift=1.75pt}] (D) to node {$11$} (A);


\end{scope}




\begin{scope}[shift={(2,2)}]
\node[inner sep=0,outer sep=1] (A) at (0,0)  {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (B) at (1,0) {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (C) at (1,1) {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (D) at (0,1) {\large \blue{$\bullet$}};

\draw[arrows={-stealth},very thick,blue,above, transform canvas={yshift=1.75pt}] (A) to node {$11$} (B);
\draw[arrows={-stealth},very thick,blue,below, transform canvas={yshift=-1.75pt}] (B) to node {$2$} (A);

\draw[arrows={-stealth},very thick,blue,left, transform canvas={xshift=-1.75pt}] (B) to node {$1$} (C);
\draw[arrows={-stealth},very thick,blue,right, transform canvas={xshift=1.75pt}] (C) to node {$1$} (B);

\draw[arrows={-stealth},very thick,blue,above, transform canvas={yshift=1.75pt}] (D) to node {$1$} (C);
\draw[arrows={-stealth},very thick,blue,below, transform canvas={yshift=-1.75pt}] (C) to node {$1$} (D);

\draw[arrows={-stealth},very thick,blue,left, transform canvas={xshift=-1.75pt}] (A) to node {$11$} (D);
\draw[arrows={-stealth},very thick,blue,right, transform canvas={xshift=1.75pt}] (D) to node {$2$} (A);

\end{scope}




\begin{scope}[shift={(0,2)}]
\node[inner sep=0,outer sep=1] (A) at (0,0)  {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (B) at (1,0) {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (C) at (1,1) {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (D) at (0,1) {\large \blue{$\bullet$}};

\draw[arrows={-stealth},very thick,blue,above, transform canvas={yshift=1.75pt}] (A) to node {$2$} (B);
\draw[arrows={-stealth},very thick,blue,below, transform canvas={yshift=-1.75pt}] (B) to node {$11$} (A);

\draw[arrows={-stealth},very thick,blue,left, transform canvas={xshift=-1.75pt}] (B) to node {$11$} (C);
\draw[arrows={-stealth},very thick,blue,right, transform canvas={xshift=1.75pt}] (C) to node {$2$} (B);

\draw[arrows={-stealth},very thick,blue,above, transform canvas={yshift=1.75pt}] (D) to node {$1$} (C);
\draw[arrows={-stealth},very thick,blue,below, transform canvas={yshift=-1.75pt}] (C) to node {$1$} (D);

\draw[arrows={-stealth},very thick,blue,left, transform canvas={xshift=-1.75pt}] (A) to node {$1$} (D);
\draw[arrows={-stealth},very thick,blue,right, transform canvas={xshift=1.75pt}] (D) to node {$1$} (A);

\end{scope}




\begin{scope}[shift={(1,1)}]
\node[inner sep=0,outer sep=1] (A) at (0,0)  {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (B) at (1,0) {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (C) at (1,1) {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (D) at (0,1) {\large \blue{$\bullet$}};

\draw[arrows={-stealth},very thick,blue,above, transform canvas={yshift=1.75pt}] (A) to node {$1$} (B);
\draw[arrows={-stealth},very thick,blue,below, transform canvas={yshift=-1.75pt}] (B) to node {$1$} (A);

\draw[arrows={-stealth},very thick,blue,left, transform canvas={xshift=-1.75pt}] (A) to node {$1$} (D);
\draw[arrows={-stealth},very thick,blue,right, transform canvas={xshift=1.75pt}] (D) to node {$1$} (A);

\draw[arrows={-stealth},very thick,blue,above, transform canvas={yshift=1.75pt}] (D) to node {$1$} (C);
\draw[arrows={-stealth},very thick,blue,below, transform canvas={yshift=-1.75pt}] (C) to node {$1$} (D);

\draw[arrows={-stealth},very thick,blue,left, transform canvas={xshift=-1.75pt}] (B) to node {$1$} (C);
\draw[arrows={-stealth},very thick,blue,right, transform canvas={xshift=1.75pt}] (C) to node {$1$} (B);

\end{scope}


%%%%%%%% START OF THE BOUNDARY EDGES


\node[inner sep=0,outer sep=1] (A1) at (1,0)  {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (A2) at (2,0)  {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (B1) at (3,1) {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (B2) at (3,2) {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (C1) at (1,3) {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (C2) at (2,3) {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (D1) at (0,1) {\large \blue{$\bullet$}};
\node[inner sep=0,outer sep=1] (D2) at (0,2) {\large \blue{$\bullet$}};

\draw[arrows={-stealth},very thick,blue,above, transform canvas={yshift=1.75pt}] (A1) to node {$1$} (A2);
\draw[arrows={-stealth},very thick,blue,below, transform canvas={yshift=-1.75pt}] (A2) to node {$1$} (A1);

\draw[arrows={-stealth},very thick,blue,left, transform canvas={xshift=-1.75pt}] (B1) to node {$1$} (B2);
\draw[arrows={-stealth},very thick,blue,right, transform canvas={xshift=1.75pt}] (B2) to node {$1$} (B1);

\draw[arrows={-stealth},very thick,blue,above, transform canvas={yshift=1.75pt}] (C1) to node {$1$} (C2);
\draw[arrows={-stealth},very thick,blue,below, transform canvas={yshift=-1.75pt}] (C2) to node {$1$} (C1);

\draw[arrows={-stealth},very thick,blue,left, transform canvas={xshift=-1.75pt}] (D1) to node {$1$} (D2);
\draw[arrows={-stealth},very thick,blue,right, transform canvas={xshift=1.75pt}] (D2) to node {$1$} (D1);






% \begin{scope}[shift={(1.5,4)}]
% \node at (0,0) {$\begin{aligned}
% \dot{x} &=  \\
% \dot{y} &= 
% \end{aligned}$};
% \end{scope}


\end{tikzpicture}
